Demystifying the Neural Tangent Kernel from a Practical Perspective: Can it be trusted for Neural Architecture Search without training?

In Neural Architecture Search (NAS), reducing the cost of architecture evaluation remains one of the most crucial challenges. Among a plethora of efforts to bypass training of each candidate architecture to convergence for evaluation, the Neural Tangent Kernel (NTK) is emerging as a promising theoretical framework that can be utilized to estimate the performance of a neural architecture at initialization. In this work, we revisit several at-initialization metrics that can be derived from the NTK and reveal their key shortcomings. Then, through the empirical analysis of the time evolution of NTK, we deduce that modern neural architectures exhibit highly non-linear characteristics, making the NTK-based metrics incapable of reliably estimating the performance of an architecture without some amount of training. To take such non-linear characteristics into account, we introduce Label-Gradient Alignment (LGA), a novel NTK-based metric whose inherent formulation allows it to capture the large amount of non-linear advantage present in modern neural architectures. With minimal amount of training, LGA obtains a meaningful level of rank correlation with the post-training test accuracy of an architecture. Lastly, we demonstrate that LGA, complemented with few epochs of training, successfully guides existing search algorithms to achieve competitive search performances with significantly less search cost. The code is available at: https://github.com/nutellamok/DemystifyingNTK.

==> tex/related_works.tex <==
\section{Related Works}
\subsection{Neural Tangent Kernel}
While research into how and what DNNs learn is at a rather premature stage, the NTK framework, first conceptualized by Jacot~\textit{et al.}~\cite{jacot2018neural}, has drawn a considerable amount of attention among Deep Learning theorists.
At least in a infinite width limit with a proper initialization scheme and a small learning rate, the NTK framework provides a solid theoretical foothold for understanding the training dynamics of DNNs.


\subsection{Neural Architecture Search}
In early NAS, evolutionary algorithm (EA)~\cite{real2017large, real2019regularized} or reinforcement learning (RL)~\cite{le2017naswithRL, zoph2018nasnet, raskar2016metaqnn} were two popular choices of search algorithm.
Although these early works were successful in proving the potential of NAS, their immediate application was challenging due to the enormous search cost, easily mounting up to tens of thousands of GPU hours to search for a single architecture.
Most of the computational overhead in early NAS algorithms occurred as the result of having to train each candidate architecture to convergence and evaluate it.

Through weight sharing~\cite{dean2018enas}, recent NAS works were able to achieve a noticeable acceleration in the architecture search process.
Weight sharing utilizes a super-network, whose sub-networks correspond to candidate architectures belonging in the pre-defined search space.
The sub-networks are evaluated with the weights inherited from the super-network, and thus, the sub-networks end up sharing a common set of weights.
Modern NAS algorithms that exploit such performance approximation techniques can be categorized into differentiable NAS~\cite{yang2019darts, chen2020stabilizing, xu2019pc, zela2019understanding, chu2019fairdarts, chen2019progressive, li2020sgas, zhou2020NAS, chu2020darts, chen2020drnas}, and one-shot NAS~\cite{le2018oneshot, dong2019searching, brock2018smash, peng2020cream, zhang2020overcoming}; while the search and evaluation processes are entangled in the former, the latter disentangles them into separate processes.
% Although weight-sharing is effective at reducing the computational cost, it often causes NAS algorithms to derive a sub-optimal architecture.

Performance predictors~\cite{deng2017peephole}, which take an encoded neural architecture as an input and output the accuracy of the corresponding architecture, are another promising direction for reducing the architecture evaluation cost.
The main challenge in performance prediction is minimizing the number of architecture-accuracy pairs required to obtain a performance predictor that generalizes well to the rest of the search space.
% Because the most straightforward way of encoding neural architectures is through directed acyclic graphs, most of the predictors employ a graph neural network as their backbone.
Because the problem of architecture performance prediction is by definition a regression task,~\cite{deng2017peephole, tang2020semi, li2020gp} aimed to predict the exact value of accuracy by minimizing the mean squared error loss between the predicted and true accuracy. 
Recently, architecture comparators~\cite{xu2021renas, chen2021contrastive}, are rising in popularity.
Instead of estimating the exact accuracy, comparators take two architectures as an input and use a ranking loss or a contrastive learning framework to predict which is more likely to rank higher in terms of accuracy.
Apart from weight sharing and performance predictors, there also exist works that aim to search for more general proxy settings for architecture evaluation~\cite{na2021accelerating, zhou2020econas}.

Our work is most closely related to NAS approaches that aim to score architectures at initialization without any amount of training.
Through a series of empirical investigation, Abdelfattah~\textit{et al.}~\cite{abdelfattah2020zero} demonstrate how effective pre-existing pruning-at-initialization techniques are at approximating the final test accuracy of architectures.
% which one of the pruning-at-initialization techniques is most useful for NAS.
The approach of NASWOT~\cite{mellor2021neural} stems from an intuition that if the feature maps generated by a single DNN from two different inputs overlap much with each other, it will be more challenging for the DNN to learn to distinguish those inputs.
NASWOT thus uses the Hamming distance between two feature maps 
binary codes—induced by the untrained network at two
inputs—as a measure of how dissimilar the two inputs are.
and proposes to score architectures based on 
KNAS~\cite{xu2021knas}, TE-NAS~\cite{chen2020neural} Zen-NAS~\cite{lin2021zen}. White~\textit{et al.}~\cite{white2021powerful}
